PanopticQuery: Unified Query-Time Reasoning for 4D Scenes

Understanding dynamic 4D environments through natural language queries requires not only accurate scene reconstruction but also robust semantic grounding across space, time, and viewpoints. While recent methods using neural representations have advanced 4D reconstruction, they remain limited in contextual reasoning, especially for complex semantics such as interactions, temporal actions, and spatial relations. A key challenge lies in transforming noisy, view-dependent predictions into globally consistent 4D interpretations. We introduce PanopticQuery, a framework for unified query-time reasoning in 4D scenes. Our approach builds on 4D Gaussian Splatting for high-fidelity dynamic reconstruction and introduces a multi-view semantic consensus mechanism that grounds natural language queries by aggregating 2D semantic predictions across multiple views and time frames. This process filters inconsistent outputs, enforces geometric consistency, and lifts 2D semantics into structured 4D groundings via neural field optimization. To support evaluation, we present Panoptic-L4D, a new benchmark for language-based querying in dynamic scenes. Experiments demonstrate that PanopticQuery sets a new state of the art on complex language queries, effectively handling attributes, actions, spatial relationships, and multi-object interactions. A video demonstration is available in the supplementary materials.

==> picture/vis3/buckets/buckets_jpg.tex <==
% ==============================================
% 颜色与基础设置
% ==============================================
\definecolor{bgA}{RGB}{223, 241, 215} 
\definecolor{bgB}{RGB}{219, 236, 249} 
\definecolor{bgC}{RGB}{255, 235, 235} 

% 路径 (保持不变)
\newcommand{\basepathC}{picture/vis3/buckets/the_bucket_between_the_red_and_blue_buckets_jpg/}
\newcommand{\basepathD}{picture/vis3/buckets/the_bucket_which_is_lifted_by_the_woman_in_pink_jpg/}


% ==============================================
% 【核心修复】统一度量衡
% ==============================================
% 计算右侧组图中单张图片的实际宽度：
% minipage宽度(0.435) * 图片比例(0.24) ≈ 0.1044
\setlength{\myImgW}{0.1044\textwidth} 

\begin{figure*}[t]
    \centering
    % 布局结构保持不变
    
    % --- 第一列：RGB ---
    \begin{minipage}[t]{0.11\linewidth}
        % 这里的 width=\linewidth 让背景保持“胖胖的” (0.11\textwidth)
        \begin{groupbox}[width=\linewidth, colback=bgC, arc=2mm]{bgC}
            \centering
            Input
            \setlength{\tabcolsep}{0pt} 
            \renewcommand{\arraystretch}{0.6}
            
            \begin{tabular}{c}
                % 占位符，保证文字行高度一致
                \phantom{ 3D} \\ 
                % 图片会自动居中，因为外层有 \centering
                \imgRGB{\basepathC frame_0001.jpg} \\
                \imgRGB{\basepathC frame_0033.jpg} \\
                \imgRGB{\basepathC frame_0065.jpg} \\
                \imgRGB{\basepathC frame_0097.jpg} 
            \end{tabular}
        \end{groupbox}
    \end{minipage}
    \hfill 
    % --- 第二列：Group A ---
    \begin{minipage}[t]{0.435\linewidth}
        \begin{groupbox}{bgA}
            \centering
            % \titleBox{a. The bucket between the red and blue buckets} \\
            Q1: The bucket between the red and blue buckets

            \setlength{\tabcolsep}{0.5pt} 
            \renewcommand{\arraystretch}{0.5} 
            
            \begin{tabular}{cccc}
                 LangSplat &  4D LangSplat &  Ours &  GT \\
                \imgCell{\basepathC d3_0.jpg} & \imgCell{\basepathC d4_0.jpg} & \imgCell{\basepathC pred_0.jpg} & \imgCell{\basepathC gt_0.jpg} \\
                \imgCell{\basepathC d3_32.jpg} & \imgCell{\basepathC d4_32.jpg} & \imgCell{\basepathC pred_32.jpg} & \imgCell{\basepathC gt_32.jpg} \\
                \imgCell{\basepathC d3_64.jpg} & \imgCell{\basepathC d4_64.jpg} & \imgCell{\basepathC pred_64.jpg} & \imgCell{\basepathC gt_64.jpg} \\
                \imgCell{\basepathC d3_96.jpg} & \imgCell{\basepathC d4_96.jpg} & \imgCell{\basepathC pred_96.jpg} & \imgCell{\basepathC gt_96.jpg} \\
            \end{tabular}
        \end{groupbox}
    \end{minipage}
    \hfill 
    % --- 第三列：Group B ---
    \begin{minipage}[t]{0.435\linewidth}
        \begin{groupbox}{bgB}
            \centering
            % \titleBox{b. The bucket which is lifted by the woman in pink} \\
            Q2: The bucket which is lifted by the woman in pink
            
            \setlength{\tabcolsep}{0.5pt} 
            \renewcommand{\arraystretch}{0.5} 
            
            \begin{tabular}{cccc}
                 LangSplat &  4D LangSplat &  Ours &  GT \\
                \imgCell{\basepathD d3_0.jpg} & \imgCell{\basepathD d4_0.jpg} & \imgCell{\basepathD pred_0.jpg} & \imgCell{\basepathD gt_0.jpg} \\
                \imgCell{\basepathD d3_32.jpg} & \imgCell{\basepathD d4_32.jpg} & \imgCell{\basepathD pred_32.jpg} & \imgCell{\basepathD gt_32.jpg} \\
                \imgCell{\basepathD d3_64.jpg} & \imgCell{\basepathD d4_64.jpg} & \imgCell{\basepathD pred_64.jpg} & \imgCell{\basepathD gt_64.jpg} \\
                \imgCell{\basepathD d3_96.jpg} & \imgCell{\basepathD d4_96.jpg} & \imgCell{\basepathD pred_96.jpg} & \imgCell{\basepathD gt_96.jpg} \\
            \end{tabular}
        \end{groupbox}
    \end{minipage}
    \vspace{-3mm}
    \caption{Qualitative Comparison on scene Bucket.}
    \label{fig:supp_qualitative_bucket}
\end{figure*}

==> picture/vis3/cook/cook_jpg.tex <==
% ==============================================
% 颜色与基础设置
% ==============================================
\definecolor{bgA}{RGB}{223, 241, 215} 
\definecolor{bgB}{RGB}{219, 236, 249} 
\definecolor{bgC}{RGB}{255, 235, 235} 

% 路径 (保持不变)
\newcommand{\basepathI}{picture/vis3/cook/the_man_cooking_jpg/}
\newcommand{\basepathJ}{picture/vis3/cook/the_pot_being_used_by_the_man_to_cook_spinach_jpg/}


% ==============================================
% 【核心修复】统一度量衡
% ==============================================
% 计算右侧组图中单张图片的实际宽度：
% minipage宽度(0.435) * 图片比例(0.24) ≈ 0.1044
\setlength{\myImgW}{0.1044\textwidth} 

\begin{figure*}[t]
    \centering
    % 布局结构保持不变
    
    % --- 第一列：RGB ---
    \begin{minipage}[t]{0.11\linewidth}
        % 这里的 width=\linewidth 让背景保持“胖胖的” (0.11\textwidth)
        \begin{groupbox}[width=\linewidth, colback=bgC, arc=2mm]{bgC}
            \centering
            % \titleBox{RGB} \\
            Input
            \setlength{\tabcolsep}{0pt} 
            \renewcommand{\arraystretch}{0.6}
            
            \begin{tabular}{c}
                % 占位符，保证文字行高度一致
                \phantom{ 3D} \\ 
                % 图片会自动居中，因为外层有 \centering
                \imgRGB{\basepathI 0000.jpg} \\
                \imgRGB{\basepathI 0080.jpg} \\
                \imgRGB{\basepathI 0160.jpg} \\
                \imgRGB{\basepathI 0240.jpg} 
            \end{tabular}
        \end{groupbox}
    \end{minipage}
    \hfill 
    % --- 第二列：Group A ---
    \begin{minipage}[t]{0.435\linewidth}
        \begin{groupbox}{bgA}
            \centering
            % \titleBox{a. The man cooking} \\
            Q1: The man cooking
            
            \setlength{\tabcolsep}{0.5pt} 
            \renewcommand{\arraystretch}{0.5} 
            
            \begin{tabular}{cccc}
                 LangSplat &  4D LangSplat &  Ours &  GT \\
                \imgCell{\basepathI d3_0.jpg} & \imgCell{\basepathI d4_0.jpg} & \imgCell{\basepathI pred_0.jpg} & \imgCell{\basepathI gt_0.jpg} \\
                \imgCell{\basepathI d3_80.jpg} & \imgCell{\basepathI d4_80.jpg} & \imgCell{\basepathI pred_80.jpg} & \imgCell{\basepathI gt_80.jpg} \\
                \imgCell{\basepathI d3_160.jpg} & \imgCell{\basepathI d4_160.jpg} & \imgCell{\basepathI pred_160.jpg} & \imgCell{\basepathI gt_160.jpg} \\
                \imgCell{\basepathI d3_240.jpg} & \imgCell{\basepathI d4_240.jpg} & \imgCell{\basepathI pred_240.jpg} & \imgCell{\basepathI gt_240.jpg} \\
            \end{tabular}
        \end{groupbox}
    \end{minipage}
    \hfill 
    % --- 第三列：Group B ---
    \begin{minipage}[t]{0.435\linewidth}
        \begin{groupbox}{bgB}
            \centering
            % \titleBox{b. The pot being used by the man to cook spinach} \\
            Q2: The pot being used by the man to cook spinach
            
            \setlength{\tabcolsep}{0.5pt} 
            \renewcommand{\arraystretch}{0.5} 
            
            \begin{tabular}{cccc}
                 LangSplat &  4D LangSplat &  Ours &  GT \\
                \imgCell{\basepathJ d3_0.jpg} & \imgCell{\basepathJ d4_0.jpg} & \imgCell{\basepathJ pred_0.jpg} & \imgCell{\basepathJ gt_0.jpg} \\
                \imgCell{\basepathJ d3_80.jpg} & \imgCell{\basepathJ d4_80.jpg} & \imgCell{\basepathJ pred_80.jpg} & \imgCell{\basepathJ gt_80.jpg} \\
                \imgCell{\basepathJ d3_160.jpg} & \imgCell{\basepathJ d4_160.jpg} & \imgCell{\basepathJ pred_160.jpg} & \imgCell{\basepathJ gt_160.jpg} \\
                \imgCell{\basepathJ d3_240.jpg} & \imgCell{\basepathJ d4_240.jpg} & \imgCell{\basepathJ pred_240.jpg} & \imgCell{\basepathJ gt_240.jpg} \\
            \end{tabular}
        \end{groupbox}
    \end{minipage}
    \vspace{-3mm}
    \caption{Qualitative Comparison on scene Cook Spinach.}
    \label{fig:supp_qualitative_cook}
\end{figure*}

==> table/ablation_seg_backbone.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on different backbones. We compare our \textit{samwise} approach with other vision-language and segmentation backbones across four query types.}
\vspace{-3mm}
\label{tab:ablation_backbone}

\setlength{\tabcolsep}{1.2pt} 

\resizebox{\columnwidth}{!}{
    
    \begin{tabular}{lcccccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{2}{c}{\textbf{Attr. Query}} & \multicolumn{2}{c}{\textbf{Act. Query}} & \multicolumn{2}{c}{\textbf{Spat. Query}} & \multicolumn{2}{c}{\textbf{Inter. Query}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & mAcc & mIoU & mAcc & mIoU & mAcc & mIoU & mAcc & mIoU \\
    \midrule

    \rowcolor{gray!20}
    Qwen2-VL (bbox) + SAM2 & 52.67 & 45.54 & 35.77 & 25.86 & 32.48 & 24.18 & 21.02 & 17.36 \\
    
    SAM3 & 75.98 & \textbf{68.81} & 60.29 & 55.27 & 60.12 & 55.91 & 34.77 & 29.10 \\

    \midrule 

    \rowcolor{gray!20}
    \textbf{SAMwise (Ours)} & \textbf{76.72} & 67.11 & \textbf{83.66} & \textbf{74.15} & \textbf{81.19} & \textbf{72.52} & \textbf{69.83} & \textbf{62.33} \\
    \bottomrule
    \end{tabular}
}
\vspace{-3mm}
\end{table}
